VioLA: Aligning Videos to 2D LiDAR Scans

We study the problem of aligning a video that captures a local portion of an environment to the 2D LiDAR scan of the entire environment. We introduce a method (VioLA) that starts with building a semantic map of the local scene from the image sequence, then extracts points at a fixed height for registering to the LiDAR map. Due to reconstruction errors or partial coverage of the camera scan, the reconstructed semantic map may not contain sufficient information for registration. To address this problem, VioLA makes use of a pre-trained text-to-image inpainting model paired with a depth completion model for filling in the missing scene content in a geometrically consistent fashion to support pose registration. We evaluate VioLA on two real-world RGB-D benchmarks, as well as a self-captured dataset of a large office scene. Notably, our proposed scene completion module improves the pose registration performance by up to 20%.

==> sections/notes.tex <==
To decide whether we should perform scene completion, we devised a decision criterion which effectively finds out if there are multiple global minima after we search for the transformation between V and L. Specifically, we consider candidate transformations and check if there are two transformations which have small error and at the same time, are not very close. The notion of closeness is associated with the rotation and translation components of the two transforms. We define T_i and T_j to be close if ..

More concretely, we start with the transform T_1 with the smallest cost after the search. We then remove its neighbors which are close from consideration and pick the second best transform T_2. Let L_1 and L_2 be the loss values associated with T_1 and T_2 respectively. If these two transforms have similar loss values (i.e. |L1-L2| < c), then it means we have multiple global minima.  





--------------
Algorithm: Scene Completion Activation
Input: 
{T_i}: sorted in ascending order according to L_i = cost(T_i)
c : user defined proximity threshold

L_1 = cost(T_1)
L_2 = min_j {cost(T_j) : T_j not close to T_1}

return |L_2-L1| < c

At a high-level, our view selection strategy first finds occlusion boundaries between observed and unobserved pixels. Then we move the camera to increase the number of unobserved pixels while maintaining a certain amount of observed pixels in the field of view. We further rotate the camera along the gravity direction to cover more unobserved pixels. Details are as follows.

First, we define four types of point sets that are used for placing the virtual cameras. a) The boundary point represented as a point at the RVC height, b) the 2D ray cast hit points at the RVC height obtained from Section~\ref{sec:ray_cast}, c) \textit{downprojected points} where we collapse all reconstructed points onto a plane at the RVC height from the top-down view, and d) \textit{keypoints} at the RVC height which approximately represent the missing parts to be completed. 

We are interested in placing the keypoints such that when the generated virtual camera trajectory tracks along these keypoints, it also gradually covers the missing part extending from the seen part. Therefore, we need to first find the boundary point that lies on the boundary of the seen part and the missing area. To do so, we remove the downprojected points that have ray cast hit points in their neighborhood. Then, the boundary point is the point in the ray cast hit points that is closest to the remaining downprojected points. Next, to place to keypoints, we fit a concave hull~\cite{duckham2008efficient,moreira2007concave} on the downprojected points and sample points on the hull boundary extending from the occlusion boundary towards the direction where there is no ray cast hit points for $2$m.

Finally, to generate the virtual camera trajectory, we first search among all the frames in the video to find the cameras that see the boundary point and pick the one with least pitch angle (i.e., camera looking down) as the first camera. Then we move the camera back along the camera's $z$-axis with a step size of $0.2$m until it sees half of the keypoints, then apply rotation about the floor normal direction with a step size of $10^{\circ}$ until it sees all the keypoints or it reaches the maximum rotation threshold ($30^{\circ}$). As shown in \figref{fig:viewpoint_simple}, these sequential viewpoints are later used in the point cloud completion module.


% We are interested in finding the target camera that sees the occlusion boundary such that both the observed and unobserved pixels are maximized in the field of view. 

% Finally, we start from the target camera position and sequentially record the following trajectory:


The boundary point: a point at the RVC height that represents the boundary of the seen part and the missing area.


%%% yet another attempt

c) \emph{keypoints}: a set of points at the RVC height that determine the largest missing area to be completed 
d) \emph{boundary point}: the point in H that's closest to the keypoints

The key idea of our strategy for viewpoint selection is to \emph{gradually} add 3D content from a sequence of virtual views. 
To achieve this, it first finds

our view selection involves multiple heuristic steps. Let us first give a high-level description. First, it identifies regions that are already observed at the RVC height. This can be done by examining non-floor points projected onto the 2D plane (Refer the figure). Once the regions are found, we may pick one region with the largest number of points. The next step is to determine an 'edge point' of the observed region, which will be a starting point to generate virtual keypoints in the unobserved area adjacent to it. Also a video frame is selected among all observed frames covering the 'edge point', which will serve as the starting camera pose for the virtual views. The last step is to generate a sequence of the camera poses that increasingly covers the keypoints as well as a good overlap of the observed region.

